Interface Design to Mitigate Inflation in Recommender Systems

Recommendation systems rely on user-provided data to learn about item quality and provide personalized recommendations. An implicit assumption when aggregating ratings into item quality is that ratings are strong indicators of item quality. In this work, we test this assumption using data collected from a music discovery application. Our study focuses on two factors that cause rating inflation: heterogeneous user rating behavior and the dynamics of personalized recommendations. We show that user rating behavior substantially varies by user, leading to item quality estimates that reflect the users who rated an item more than the item quality itself. Additionally, items that are more likely to be shown via personalized recommendations can experience a substantial increase in their exposure and potential bias toward them. To mitigate these effects, we analyze the results of a randomized controlled trial in which the rating interface was modified. The test resulted in a substantial improvement in user rating behavior and a reduction in item quality inflation. These findings highlight the importance of carefully considering the assumptions underlying recommendation systems and designing interfaces that encourage accurate rating behavior.

==> motivation.tex <==
\section{Natural experiment: introduction of timers}
\label{sec:natural_exp}


% We examined the mean rating of users over a period of 16 months (between January 2020 and May 2022).
% Figure~\ref{fig:split_corr} shows the correlation between the mean user rating in two consecutive months along with confidence intervals here, via bootstrapping, and users with ratings less than the $20^{th}$ percentile of ratings ($7$ ratings) are excluded.
% The correlation decreases the most in January 2021, which is when the interface was changed.






% 1. Users heterogeneous
% 2. A function of user more than songs
% 3. User interface tunes both of these things.






% \begin{figure}[h]
% \centering
% % \includegraphics[scale=0.5]{graphs/natural_exp/Mean ratio per rating type.png}
% \includegraphics[scale=0.5]{plots_nikhil/naturalexperiment_ratings_distribution.pdf}
% \caption{Mean ratings of each option (dislikes, likes and superlikes) before and after change.}
% \label{fig:mean_rating_before_after}
% \end{figure}



% \begin{figure}[h]
% \centering
% % \includegraphics[scale=0.5]{graphs/natural_exp/Mean user score histogram.png}
% \includegraphics[scale=0.5]{plots_nikhil/naturalexperiment_histogram_user_scores.pdf}
% \caption{Mean user score}
% \label{fig:user_score_hist}
% \end{figure}







% \input{plots_nikhil/naturalexperiment_likeregression.tex}

% \begin{table}[th]
% 	\begin{center}
% 		\begin{tabular}{p{3cm}|p{1cm} |p{1cm}|p{2cm}|p{1cm} |p{1cm} }
% 			\toprule
% 			R-squared & $0.206$ & & & & \\
%             \midrule
%             & coef & t & $P > [t]$ & $0.025$ & $0.975$ \\
% 			\midrule
% 			const & $0.1345$ & $28.316$ & $0.000$ & $0.125$ & $0.144$\\
% 			\midrule
%             mean user factor & $0.2812$& $59.839$& $0.000$& $0.272$& $0.290$ \\
% 			\midrule
%             song factor & $0.3533$& $34.383$& $0.000$& $0.333$& $0.373$ \\
%             \bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{Pre change regression table}
% 	\label{tab:pre_change}
% \end{table}




% \begin{table}[th]
% 	\begin{center}
% 		\begin{tabular}{p{3cm}|p{1cm} |p{1cm}|p{2cm}|p{1cm} |p{1cm} }
% 			\toprule
% 			R-squared & $0.343$ & & & & \\
%             \midrule
%             & coef & t & $P > [t]$ & $0.025$ & $0.975$ \\
% 			\midrule
% 			const & $-0.0615$ & $-10.608$ & $0.000$ & $-0.073$ & $-0.050$\\
% 			\midrule
%             mean user factor & $0.3460$& $63.370$& $0.000$& $0.335$& $0.357$ \\
% 			\midrule
%             song factor & $1.1274$& $112.434$& $0.000$& $1.108$& $1.147$ \\
%             \bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{Post change regression table}
% 	\label{tab:post_change}
% \end{table}





% The reduction indicates that the mean rating per user was influenced by the interface modification, and as a result, it motivated the experiment detailed below.




%Our work focuses on whether we can improve the platform interface design in such a way that it incentivizes users to give real trinary ratings to songs that are aligned with their individual tastes, thus limiting the super-like and pickiness phenomena among users which resulting in quality data.





%TODO: add limitation of the natural experiment
%TODO: Limitations about platform/what is missing from before/after
%Limitation: low traffic in months adjacents to the modifications
% overlap users number was low
%overall users number low
% can't analyze personalied since algorithms changed

%TODO: what will be learned from an actual experiment


